Split Localized Conformal Prediction

Conformal prediction is a simple and powerful tool that can quantify uncertainty without any distributional assumptions. Many existing methods only address the average coverage guarantee, which is not ideal compared to the stronger conditional coverage guarantee. Existing methods of approximating conditional coverage require additional models or time effort, which makes them not easy to scale. In this paper, we propose a modified non-conformity score by leveraging the local approximation of the conditional distribution using kernel density estimation. The modified score inherits the spirit of split conformal methods, which is simple and efficient and can scale to high dimensional settings. We also proposed a unified framework that brings together our method and several state-of-the-art. We perform extensive empirical evaluations: results measured by both average and conditional coverage confirm the advantage of our method.

==> tex/backup.tex <==
\subsection{Quantile Regression and Conditional Coverage}
\qq{how is this related the last section? We need to construct $\hat\mu$...}
The goal for\qq{of} conditional quantile regression\citep{koenker1978regression}
is to estimate the quantile of $Y$ given random variable $X=x$.
Let $F(\cdot|X=x)$ be the condition distribution or the cumulative function defined as
$$
    F(y|X=x) = \P(Y\leq y|X=x),
$$
and its $\alpha th$\qq{$\alpha$-th} conditional quantile function is defined as:
$$
    q_\alpha(x) := \inf \{y\in \R:~F(y|X=x)\geq \alpha\}.
$$

If we get access to the conditional quantile function $q_\alpha(x)$, fix\qq{ing}
$\alo = \frac{\alpha}{2}$ and $\ahi = 1-\frac{\alpha}{2}$ and set\qq{ing}
\begin{equation}\label{eqn:oracle_band}
    \C^{\rm oracle}(x) = [q_{\alo}(x), q_{\ahi}(x)],
\end{equation}
we can achieve \textit{conditional coverage} guarantee 
\begin{equation}\label{eqn:conditional_coverage}
    \P(Y_{n+1}\in \C(x)|X_{n+1}=x) \geq 1-\alpha,
\end{equation}
\qq{we should discuss the difference of average (marginal) vs. conditional coverage. It is an important difference.}
if we set $\C = \C^{\rm oracle}$.

% Actually the inequality in Eq.~\eqref{eqn:conditional_coverage} can be replaced by equality
% $$
%     \P(Y_{n+1}\in C^{\rm oracle}(x)|X_{n+1}=x) = 1-\alpha.
% $$

\ziyang{-->add the heteroskedascity example here? mention the advantage of conditonal coverage compared with average coverage.}

\begin{figure}
    \centering
    \includegraphics[width = 0.3\textwidth]{fig/pinball.pdf}
    \caption{Illustration of pinball loss}
    \label{fig:pinball}
\end{figure}

\subsection{Estimating the Conditional Quantile Function}

\qq{how are the two methods connnected / interact? why introduce both of them? need specify; give an overview }

\myparagraph{Parametric Estimation as an Optimization Problem \qq{sounds too obvious? do you mean quantile estimation via optimization?}}
The most classical way of estimating the conditional quantile function
can be cast as an optimization problem:
\begin{equation}\label{eqn:parametric_q_alpha}
    \hat{q}_{\alpha}(x) = f_{\hat{\theta}}(x), \qquad \hat{\theta} = \argmin_{\theta} \sum_{i\in \I_{train}} \rho_\alpha(Y_i, f_{\theta}(X_i)) + \R(\theta),
\end{equation}
\qq{define $f_\theta$}
where $\R(\theta)$\qq{$\R$ may be reserved for real numbers} is the regularization of parameter $\theta$ 
and the "pinball loss" $\rho_\alpha$(Figure~\ref{fig:pinball}) is defined as:
$$
    \rho_\alpha(y,\hat{y}) = \alpha(y-\hat{y})\mathds{1}_{y>\hat{y}} + (1-\alpha)(\hat{y}-y)\mathds{1}_{y\leq \hat{y}}.
$$
Equipped with universal approximator\qq{s} such as deep neural network\qq{mapping back to the set of $f_\theta$},
the estimation $\hat{q}_{\alpha}$ can approximate $q_\alpha(x)$ well
and is widely used in many areas.

\myparagraph{Non-Parametric Estimation: Local Linear Quantile Regression}
From the definition of condition quantile \qq{functions?}, we can see that 
\qq{the} condition distribution\qq{addspace}(cumulative function) is important for estimating
the quantile function\qq{it is obviously important?}.
The Non-parametric way of estimating quantile regression\citep{yu1998local,hall1999methods}\qq{quantile regression is not something can to be estimated?} 
is by computing the empirical quantile of its 
kernel smoothing conditional distribution from the data.

More specifically, define:
$$
    \hat{F}_h(y|X=x) = \sum_{i\in \I_{train}} w_h(X_i|x)\mathds{1}_{y\leq Y_i},
$$
where $w_h(X_i|x) = \frac{K(\frac{\|X_i-x\|}{h})}{\sum_{j\in \I_{train}}K(\frac{\|X_j-x\|}{h})}$ \qq{make it a single line equation}
with any kernel function $K(\cdot)$ such as boxcar kernel or Guassian Kernel.

After that, we can estimate the conditional quantile function as:
\begin{equation}\label{eqn:nonparametric_q_alpha}
    \hat{q}_{\alpha}(x) = {\rm Quantile}(\alpha, \hat{F}_h(y|X=x)),
\end{equation}
where the quantile can be easily computed by scanning all $Y_i$ and see if the empirical
cumulative weight is above $\alpha$.
Similar to other non-parametric smoothing methods, the best choice of bandwidth $h$
tradeoffs of bias and variance, which is approximately by a constant $C_\alpha$ times the 
mean distance $h_{mean}$, where $C_\alpha$ depends on the proportion value $\alpha$\citep{yu1998local}.


\subsection{Conformal Quantile Regression: Approximating Conditional Coverage with Average Coverage Guarantee}
In \qq{the} previous section, we discuss different approach\qq{s} to estimate\qq{an approach to doing (not to do) something; or an approach to something (noun)} the conditional quantile function.
Suppose we get\qq{have} access to $\hat{q}_{\alo}$ and $\hat{q}_{\ahi}$, a natural way to construct the confidence band is by set $\C$ as
$$
    \hat{\C}(x) = [\hat{q}_{\alo}(x), \hat{q}_{\ahi}(x)].
$$
However, since $\hat{q}_{\alpha},~\forall \alpha\in \{\alo, \ahi\}$ is not exact conditional quantile function, $\hat{\C}$ has no guarantee to satisfy either Eq.~\eqref{eqn:average_coverage} or Eq.~\eqref{eqn:conditional_coverage}.

Conformal quantile regression(CQR) builds confidence band on top of estimated model $\hat{q}_{\alpha}$ to satisfy average coverage guarantee.
The idea is similar to split conformal prediction, by constructing non-conformity score
$$
    E_i = \max\{\hat{q}_{\alo}(X_i)-Y_i, Y_i - \hat{q}_{\ahi}(X_i)\},~\forall i\in \I_{cal}
$$
in calibration set and compute the empirical quantile
$$
    d = {\rm Quantile}(1-\alpha, \{E_i\}_{i\in \I_{cal}}\cup \{+\infty\})
$$
as correction term, and set the condidence band as
$$
    \C_{CQR}(x) = [\hat{q}_{\alo}(x) - d, \hat{q}_{\ahi}(x) + d].
$$
Similar to split conformal prediction, CQR achieves average coverage guarantee in Eq.~\eqref{eqn:average_coverage}.

\myparagraph{Approximate Conditional Coverage}
The benefit of CQR compared with split conformal prediction is that it can approximate conditional coverage.
Once the estimated quantile model is accurate, the correction term converges to 0: $\E_{\I_{cal}}[d] = 0$\qq{what is the random variable here?}, and the confidence band will reduce back to oracle band in Eq.~\eqref{eqn:oracle_band}.

Different from \qq{the} \textit{average coverage} guarantee in Eq.~\eqref{eqn:average_coverage},
the conditional coverage is much stronger, and the distribution of $X$ can be arbitrary
so it is automatically robust to distribution free uncertainty estimation
under covariate shift\citep{tibshirani2019conformal} with arbitrary distribution on $X$:
\begin{align*}
    &\P_{X_{n+1}\sim Q_X, Y_{n+1}\sim P_{Y|X}}(Y_{n+1} \in \C(X_{n+1})) \\
    = & \sum_x \P(Y_{n+1} \in \C(x)|X_{n+1} = x) \P_{X_{n+1}\sim Q_x}(X_{n+1} = x) \\
    \geq & (1-\alpha) \sum_x \P_{X_{n+1}\sim Q_x}(X_{n+1} = x) \\
    =& 1-\alpha.
\end{align*}
\qq{no new line here; eliminate the space}
Although \citet{lei2014distribution} shows that any method satisfies Eq.~\eqref{eqn:conditional_coverage}
property must yield an interval $\C(x)$ with infinite expected length at any non-atom point $x$,
CQR in practice equipped with an almost accurate model can provide approximate conditional coverage in general.
\qq{I feel this should move to earlier when we differentiate the two guarantees.}
\qq{however, does our method achieve conditional gurantee, or some approximation of it? otherwise it is unclear why we emphasize it a lot}


\qq{i feel the intro should be re-organized.}


\begin{algorithm*}[t] 
    \caption{Conformal Quantile Regression with Localized Correction}  
    \label{alg:DDCP}
    \begin{algorithmic} 
    \STATE {\bf Input}: 
    Training Data $(X_i, Y_i)_{i=1}^n$;
    Miscoverage level $\alpha$;
    Localizer $w_h(\cdot|\cdot)$;
    \STATE {\bf Process}:\\
    1. Randomly split dataset index as $I_{train}$ and $I_{cal}$;\\
    2. Fit model with $I_{train}$ with training algorithm and get estimation: $\hat{q}_{\alo}, \hat{q}_{\ahi}$;
    We can either use mean model $\hat{q}_{\alo} = \hat{q}_{\ahi} = \hat{\mu}$ or train it seperately with pinball loss; \\
    3. Correct the quantile model with Eq.~\eqref{eqn:localized_correction} to get $\hat{q}_{\alo,h}$ and $\hat{q}_{\ahi,h}$. \\
    4. Compute $d$ using calibration $\I_{cal}$ in Eq.~\eqref{eqn:localized_d}.
    \STATE {\bf Output}:
    Conformal band $\C(x) = [\hat{q}_{\alo,h}(x)-d, \hat{q}_{\ahi,h}(x)+d]$, 
    \end{algorithmic} 
\end{algorithm*}

\section{Conformal Quantile Regression with Localized Correction}

\subsection{Quantile Regression with Localized Correction}
% Local linear quantile regression in previous section gives us a way 
% to estimate conditional quantile function leveraging local information.
The success of CQR heavily relies on the quality of the estimation of the conditional quantile model.
When the quantile model is imperfect, the performance of CQR may drop.
In the extreme case, if the two quantile models equal to the mean model, i.e. $\hat{q}_{\alo} = \hat{q}_{\ahi} = \hat{\mu}$, CQR reduces back to split conformal which provides constant length band across different location.
To address this issue,
we start with a new method that leverage the localized information 
to correct an imperfect conditional quantile model.

Suppose we get access to a fixed conditional quantile functions of $\hat{q}_{\alpha}$ 
on proportion $\alpha$, the random variable $Y$ can be viewed as a 
decomposition of two random variable:
\begin{equation}\label{eqn:decompose_Y}
    Y =  \hat{q}_{\alpha}(X) + \left(Y - \hat{q}_{\alpha}(X)\right):= \hat{q}_{\alpha}(X) + R_\alpha ,
\end{equation}
where if\qq{??} the first term $R_\alpha = R_\alpha(X,Y) := Y - \hat{q}_{\alpha}(X)$ is the residual 
and the second term is the return value of $\hat{q}_\alpha$.
Compared with the scale of $Y$, 
$R_\alpha(X,Y)$ is usually smaller once $\hat{q}_{\alpha}$ achieves the same scale as $Y$\qq{achieving the same scale is not sufficient for $ R$ to be small} \qq{achieving good approximation error; but it also depends on $alpha$, if $alpha =0,1$ it is still large.}.

Conformal quantile regression leverages $R_{\alo}$ and $R_{\ahi}$
and compute their empirical quantiles over the calibration set, 
and use them to correct the band function $\C$ so that the corrected band achieves average coverage guarantee.
However, the correction is conducted over the entire calibration set, 
which does not leverage the local information of $x$ if we want to construct $\C(x)$.

Inspired by localized conformal prediction\citep{guan2019conformal, tibshirani2019conformal} 
and the non-parametric estimation of conditional quantile function,
we can estimate the quantile of $R_\alpha|X=x$ in a non-parametric fashion and use it to correct $\hat{q}_\alpha$.

More formally, consider
\begin{equation}\label{eqn:localized_correction}
    \hat{q}_{\alpha,h}(x) = \hat{q}_{\alpha}(x) + {\rm Quantile}(\alpha, \hat{F}_h(R_\alpha=r|X=x)),
\end{equation}
where $\hat{F}_h(r|X=x) = \sum_{i\in \I_{train}} w_h(X_i|x) \mathds{1}_{r\leq Y_i-\hat{q}_{\alpha}(X_i)}$.

Compared with Eq.~\eqref{eqn:decompose_Y}, Eq.~\eqref{eqn:localized_correction} can be interpreted as estimation of quantile value of both $R_\alpha$ and $\hat{q}_{\alpha}(X)$ given $X=x$ and put them together.
Although quantile function is not linearly separable in general, the hope is that the quantile of the residual can help to correct the imperfect $\hat{q}_\alpha$ model, which can be formally expressed as the following theorem.

\qq{is the whole thing about correcting the quantile estimation? if so, we should point it very clearly}

\qq{it is still unclear why Eq 9 would be better than each individual estimator.}

\qq{i feel it will be clearer/more interesting to introduce the method from the "difference in difference" view; other than about "correcting quantile estimation" view.}

\begin{thm}\label{thm:doubly_robust}
    Define $F_h(r|X=x) = \E[w_h(X|x)\mathds{1}_{r\leq Y-\hat{q}_{\alpha}(X)}]$ as the population distribution of $\hat{F}_h$ and its corresponding population version of $\hat{q}_{\alpha,h}$ is defined as
    \begin{equation}
        q_{\alpha, h}(x) = \hat{q}_{\alpha}(x) + {\rm Quantile}(\alpha, F_h(r|X=x)),~\forall h > 0,
    \end{equation}
    we have:
    \begin{enumerate}
        \item If $\hat{q}_{\alpha} = {q}_{\alpha}$, then ${q}_{\alpha,h} = {q}_{\alpha},~\forall h>0$.
        \item The right limitation of $q_{\alpha,h}$ at point $0$ converge to $q_\alpha$:
        $$
            \lim_{h\to 0^+}{q}_{\alpha, h}(x) = {q}_{\alpha}(x),~\forall x.
        $$
    \end{enumerate}
\end{thm}

From Theorem~\ref{thm:doubly_robust} we can see that the corrected model achieves double robustness in the sense that either the model is accurate or the kernel density estimation is accurate to represent the conditional distribution, our estimator is consistent.
In practice, the correction term of empirical quantile is evaluated on finite training data, we cannot pick infinitesimal $h$ to achieve better performance since it has large variance.
Similar to kernel density estimation, the tradeoff between bias and variance can guide us the selection of the bandwidth $h$; see \citet{yu1998local} for more discussions on bandwidth selection.



\subsection{Conformal Prediction with Corrected Quantile Model}
Similar to conformal quantile regression, if we directly construct the conformal band as $\hat{\C}(x) = [\hat{q}_{\alo,h}(x), \hat{q}_{\ahi,h}(x)]$, we don't have any guarantee.
Thus, we can apply conformal quantile regression on the corrected model $\hat{q}_{\alpha, h}$.

The general procedure is straightforward.
We first divide the training dataset $(X_i,Y_i)_{i=1}^n$ randomly as two index sets $\I_{train}$ and $\I_{cal}$ such that $\I_{train}\cap \I_{cal} = \empty,~\I_{train}\cup \I_{cal} = \{1,2,\ldots,n\}$.

The next step we apply any parametric estimation algorithm $\mathcal{A}$ to get $\hat{q}_{\alo}, \hat{q}_{\ahi} \gets \mathcal{A}(\I_{train})$ from the training set.
Notice that we don't require the a perfect estimation since in the next step we will apply localized correction.
Moreover, we can even set $\hat{q}_{\alo} = \hat{q}_{\ahi} = \hat{\mu}$ as the estimated mean model, similar to split conformal prediction process. 
In experiment, we find that the drop in performance with an imperfect model is small compared with the drop in performance from CQR with perfect quantile model to split conformal prediction.

Then we apply Eq.~\eqref{eqn:localized_correction} to correct $\hat{q}_{\alo}$ and $\hat{q}_{\ahi}$ with the training data, and compute
\begin{equation*}
    E_i = \max\{\hat{q}_{\alo,h}(X_i)-Y_i, Y_i - \hat{q}_{\ahi,h}(X_i)\},~\forall i\in \I_{cal},
\end{equation*}
in calibration set, and compute
\begin{equation}\label{eqn:localized_d}
    d = {\rm Quantile}(1-\alpha, \{E_i:~i\in \I_{cal}\}\cup \{\infty\}).
\end{equation}

Finally we set our band as 
$$
    \hat{\C}(x) = [\hat{q}_{\alo,h}(x) - d, \hat{q}_{\ahi,h}(X_i) + d].
$$

We summarize the algorithmic details for the ease of reference in Algorithm~\ref{alg:DDCP}.
Similar to CQR, it is easy to show $\hat{\C}(x)$ satisfies the average coverage guarantee:
$$
    \P(Y_{n+1}\in \hat{\C}(X_{n+1})\geq 1-\alpha,
$$
and similar to CQR, we can extend to asymmetric version; see \citet{romano2019conformalized} Theorem 2 for more details.

% Given $\hat{q}_{\alo}, \hat{q}_{\ahi}$, and $(X_i, Y_i),~\forall i\in I_{train}\cup I_{cal}$.
% \begin{enumerate}
%     \item Set $V_{i,lo} = \hat{q}_{\alo}(X_i) - Y_i$, $V_{i,hi} = Y_i - \hat{q}_{\ahi}(X_i),~\forall i\in I_{train}\cup I_{cal}$.
%     \item Set 
%     \begin{align*}
%         DV_{i,lo} =& V_{i,lo} - Q(1-\alo, \sum_{j\in I_{train}}p_w(X_j|X_i) V_{j,lo}) \\
%         DV_{i,hi} =& V_{i,hi} - Q(\ahi, \sum_{j\in I_{train}}p_w(X_j|X_i) V_{j,hi}),~\forall i\in I_{cal}.
%     \end{align*}
%     \item Compute $d_i = \max\{DV_{i,lo}, DV_{i,hi}\}$, and $d = Q(1-\alpha, \{d_i\}\cup\{\infty\})$.
%     \item Set 
%     $$
%     \hat{C}(x) = [
%         \hat{q}_{\alo}(x) - Q(1-\alo, \sum_{j\in I_{train}}p_w(X_j|x) V_{j,lo}) - d,
%         \hat{q}_{\ahi}(x) + Q(\ahi, \sum_{j\in I_{train}}p_w(X_j|x) V_{j,hi}) + d]
%     $$
% \end{enumerate}


\section{Proof}
\subsection{Proof of Theorem~\ref{thm:doubly_robust}}
\begin{proof}
    \begin{enumerate}
        \item If $\hat{q}= {q}_{\alpha}$, then 
        \begin{align*}
            \Pr[Y-q_{\alpha}(x)\leq 0|X=x] = \alpha,
        \end{align*}
        which implies:
        \begin{align*}
            \sum_{x} \Pr[X=x] w_h(x|x_0)\Pr[Y-q_{\alpha}(x)\leq 0|X=x] = \alpha,
        \end{align*}
        thus
        $$
        \Q(\alpha, \E[w_h(X|x_0)\delta_{(Y-\hat{q}(X))}]) = 0.
        $$
        \item If $h\to 0$, we have:
        \begin{align*}
            &\lim_{h\to 0} \Q(\alpha, \E[w_h(X|x_0)\delta_{(Y-\hat{q}(X))}]) \\
            =& \Q(\alpha, (Y-\hat{q}(x_0)|X=x_0)]) \\
            =& \Q(\alpha, Y|X=x_0) - \hat{q}(x_0) \\
            =& q_{\alpha}(x_0) - \hat{q}(x_0).
        \end{align*}
        Therefore
        $$
            \lim_{h\to 0} q_{\alpha,h}(x_0) 
            = \hat{q}(x_0) + \left(q_{\alpha}(x_0) - \hat{q}(x_0)\right)
            = q_{\alpha}(x_0).
        $$
    \end{enumerate}
\end{proof}

\section{Decorrelation Related}

Let $\mu(x) = \E[Y|X=x]$.

Then the covariance between $Y - \mu(X)$ and $X$ becomes:
\begin{align*}
    &\E[(Y-\mu(X)) X] - \E[Y - \mu(X)]\E[X] \\
    =& \E[XY] - \E_X[\E[Y|X]X] - (\E[Y] - \E_X[\E[Y|X]])\E X \\
    =& \E[XY] - \E[XY] - (\E[Y] - \E[Y])\E[X] = 0.
\end{align*}

Therefore, if we have a approximation of $\mu(x)$, we can decorrelate $Y$ and $X$ (but not make them independent).

A localized approximation is
$$
\hat{\mu}_h(x) = \sum_{i} w_h(X_i|x) Y_i,
$$
where $w_h(X_i|x) = \frac{K(\|X_i-x\|/h)}{\sum_{j} K(\|X_j-x\|/h)}$.

Therefore, we choose $E(x,y) - \sum_{i}w_h(X_i|x) Y_i$ as the new decorrelated non-conformity score.


\paragraph{Remark}
Indepedent:
$X$ is independent to $Y$: for any function $f$ and $g$, $f(X)$ is uncorrelated to $g(Y)$.

\subsection{Another View}

Our goal:
Let
$
    \Pr[E\leq d|X=x]
$
close to
$
    \Pr[E\leq d]
$
Or
$\E[\mathds{1}_{E\leq d}|X=x]$ close to $\E[\mathds{1}_{E\leq d}]$.

Let $V = \mathds{1}_{E\leq d}$, we just need $V$ to be uncorrelated with $X$.

\section{Backup}
\section{Towards Conditional Coverage Guarantee}
\subsection{Conditional Coverage Guarantee}
\label{sec:approx_condition}
% \section{Split Localized Conformal Prediction}
% \section{Conformal Prediction with Localized Decorrelation}

% Outline
% 0. Background, split conformal, compute V= V(X,Y), do quantile lemma on V, inversely compute for Y.
% 1. When we can directly apply split conformal prediction: when distribution of V|X=x is the same for all x, introduce ideal scenario
% 2. Requires two harsh conditions: (1) exists a function V^*(X,Y) = \epsilon
%                                   (2) V = V^* exactly
% 3. It is almost imporssible, need strong assumption on distribution (for 1); exact model (for 2)
% 4. Weighted conformal -> leads to d \delta(x=x_0)/d P(x), impossible
% 5. Localized approximation by weighted conformal paper is proposed, drawback: fixed x_0, need an additional union bounds
% 6. Localized Conformal Prediction by Leying. Full conformal approach. Can also extend to \tilde{h}. Drawback: time-consuming
% 7. Out approach, move approximate quantile over training set! Do in split conformal way. Change the event to additive style (or multiplicative style).

However, we can still approximate the conditional guarantee.



\subsection{Ideal Scenario v.s. Real Scenario}


% The ideal scenario when split conformal prediction works well is when
% the non-conformity score $E = E(X,Y)$ is independent to $X$,
% Then
% \begin{align*}
%     \P(E\leq d|X=x) = \P(E\leq d),
% \end{align*}
% where the equation is due to the independence of $E$ and $X$.
% Then we can construct $\C(x) = \{y: E(x,y)\leq d\}$ and it automatically satisfies both average and conditional guarantees.

% For example, if the true underlying conditional distribution of $Y|X$ is
% $Y = \mu(X) + \varepsilon,$ where $\varepsilon$ is a zero-mean random variable that is independent of $X$. Then if the estimated mean model is exact, the non-conformity score $E = E(X,Y) = Y - \mu(X) = \varepsilon$ is independent of $X$, the event $E \leq d$ satisfies:
% $$
%     \P(E\leq d|X=x) = \P(E\leq d) \leq 1-\alpha,
% $$
% where we set $d = \Q(\alpha, \{E_i\}_{i\in \I_{cal}})$ as the empirical quantile of $E_i$ in the calibration set.
    
% \subsection{Decorrelation with Localized Difference}
% \ziyang{TODO: Rewrite the whole section}

% \ziyang{TODO: Add new theory for decorrelation}

% \ziyang{TODO: Add citation for localized decorrelation}


% In general case, it is possible that the non-conformity score $E$ is not independent of $X$,
% which can be caused by heteroscedasticity noise. Therefore,
% even when the exact mean model is obtained, $Y - \mu(X)$ will still be correlated to $X$.
% Another reason is that our estimated model on finite training data is not exact, leaving a residual $\hat{\mu}(X) - \mu(X)$ that is correlated to $X$.

Moreover, even if such mapping exists, 
finding out such mapping relies on strong distribution assumption and accurate estimation.
For example, if the true underlying distribution follows by Gaussian assumption:
$$
    Y = \mu(x) + \sigma(x) \varepsilon,
$$
where $\varepsilon\perp X$, 
we can construct $f^*(X,Y) = \frac{Y - \mu(X)}{\sigma(X)}$,
and estimate $\hat{\mu}$ and $\hat{\sigma}$ respectively \citep{lei2018distribution, papadopoulos2011regression}.
However, \citet{romano2019conformalized} states the limitation \ziyang{Add more}.
This suggests that \red{XXX}.

\subsection{Localized Conditional Coverage}
Another way to approximate conditional coverage guarantee is by weighted conformal prediction \citep{tibshirani2019conformal}, which provides guarantee when the distribution of $X$ is changed from $P(X)$ to $\tilde{P}(X)$ (covariate shift) but the conditional distribution of $Y|X$ remains the same.
From this perspective, we can view conditional coverage guarantee as changing the distribution of $X$ to a delta measure $\tilde{P}(X) = \delta(X=x_0)$ for a given $x_0$ if we care about the conditional probability when $X=x_0$: $P(Y\in \hat{\C}(X)|X=x_0)$.

However, if we follow the weighted conformal prediction and compute the density ratio we will find out that $w(x) = \frac{d \tilde{P}(x)}{d P(x)} = \frac{d \delta(x=x_0)}{d P(x)}$ is unbounded.
\citet{tibshirani2019conformal} proposes an alternative locally-smoothed approximation, which relaxes the conditional coverage as a kernel smoothing around $X=x_0$:
\begin{equation}\label{eqn:kernel_condition}
    \frac{\int \P(Y \in \C(x_0)|X = x)K(\frac{\|x-x_0\|}{h})d P(x)}{\int K(\frac{\|x-x_0\|}{h})d P(x)} \geq 1-\alpha,
\end{equation}

% Another way to approximate conditional coverage guarantee is localized conditional coverage \citep{tibshirani2019conformal}, which relaxes the conditional coverage as a kernel smoothing around $X=x$:

% \qq{did you define $P_X$?}
where $P$ is the marginal distribution of $X$ and $K(\cdot)$ can be any kernel function such as the boxcar kernel or Gaussian Kernel.
To satisfy the localized conditional coverage guarantee, we need to add a weight $w_h(X_i|x_0) \propto K(\frac{\|X_i-x_0\|}{h})$ to the non-conformity score $V_i$,
% \qq{what do you mean? move Eq 9 earlier?} 
and compute $\hat{F}_h$ as the kernel density estimation of conditional distribution of $V$ given $X=x_0$:
\begin{equation}\label{eqn:conditional_kde}
    \hat{F}_h(V=v|X=x_0) = \sum_{i\in \I_{cal}} w_h(X_i|x_0) \mathds{1}_{v\leq V_i}.
\end{equation}
Then we calculate the empirical quantile based on the weighted distribution around $x_0$:
\begin{equation}\label{eqn:kernel_d}
    d_h(x_0) = \Q(1-\alpha, \hat{F}_h(V|X=x_0))
\end{equation}
and set
the final conformal band $\C$ that satisfies the the localized conditional coverage in Eq \eqref{eqn:kernel_condition} as:
\begin{equation}\label{eqn:localized_band}
    \C(x_0) = \{y:E(x_0,y)\leq d_h(x_0)\},~{\rm satisfies}~ \eqref{eqn:kernel_condition}.
\end{equation}

In particular, if we set the non-conformity score as $V_i = |Y_i - \hat{\mu}(X_i)|$, then $$\C(x_0) = [\hat{\mu}(x_0) - d_h(x_0), \hat{\mu}(x_0) + d_h(x_0)].$$

% where the new empirical quantile need to compute with a reweight distribution of the non-conformity score.
% We will formalize it in the next section.
However, this is only valid for a given center $x_0$.
% \qq{is our method somehow equivalent to taking $x_0$ to be the training data?}.
Similar to the previously mentioned partition idea, many center points $x_0$ are needed to cover the whole domain, and one needs to divide the miscoverage rate for each center point by the total number of center points, which may yield a large interval.

\subsection{Localized Conformal Prediction}
\citet{guan2019conformal} introduces localized conformal prediction which leverages the localized distribution in Eq.~\eqref{eqn:conditional_kde} to construct a band $\C$.
The idea of localized conformal prediction is to seek an $\tilde{\alpha}$ that can satisfy the average coverage guarantee.
Instead of predefined fixed center $x_0$, let $\hat{\F_j} = \hat{\F}_h(V=v|X = X_j) = \sum_{i\in \I_{cal}}w_h(X_i|X_j) \mathds{i}_{v\leq V_i}$ as the empirical distribution centered around calibration data $X_j$.
Then consider the event 
\begin{equation}\label{eqn:event_lcb}
    E_j(\tilde{\alpha}): V_j \leq \rm{Quantile}(1-\tilde{\alpha}, \hat{\F_j}),
\end{equation}
by exchangeability, we know that
$$
    \P(E_{n+1}) \geq \E[\frac{1}{|\I_2|+1} \sum_{i\in \I_2} \mathds{1}_{E_j}(\tilde{\alpha})].
$$
Noticed that if we set $\hat{\F}_i = \hat{\F} = \frac{1}{|\I_{cal}|}\sum_{i\in \I_{cal}}\mathds{1}_{v\leq V_j}$, then if $\tilde{\alpha} = \alpha$, by quantile lemma, we will automatically satisfies
$$
    \frac{1}{|\I_2|+1} \sum_{i\in \I_2} \mathds{1}_{E_j}(\alpha) \geq 1-\alpha.
$$
However, this is not true since we change $\hat{\F}_i$ by centering around $X_i$ for each datapoint,
thus if we can inversely find $\tilde{\alpha}$ such that:
\begin{equation}\label{eqn:inverse_alpha_guarantee}
    \frac{1}{|\I_2|+1} \sum_{i\in \I_2} \mathds{1}_{E_j} \geq 1-\alpha,
\end{equation}
we can still have the coverage guarantee:
$$
    \P(V_{n+1}\leq \rm{Quantile}(1-\tilde{\alpha}, \hat{\F}(X_{n+1})) \geq 1-\alpha,
$$
where the quantile value is over the localized weighted empirical distribution around $X_{n+1}$.

In summary, the localized conformal prediction consists of two steps:
\begin{enumerate}
    \item Inversely compute $\tilde{\alpha}$ that satisfies Eq.~\eqref{eqn:inverse_alpha_guarantee}.
    \item Fit $\tilde{\alpha}$ into $\hat{C}$ as:
    \begin{equation}\label{eqn:localized_conformal}
        \hat{C}(X_{n+1}) = [\hat{\mu}(X_{n+1}) - d(X_{n+1}), \hat{\mu}(X_{n+1}) + d(X_{n+1})],
    \end{equation}
    where $d(X_{n+1}) = \rm{Quantile}(1-\tilde{\alpha}, \hat{\F}(X_{n+1}))$.
\end{enumerate}

\myparagraph{Computational Inefficient}
The major weakness of localized conformal prediction is that it is 

\subsection{Decorrelation as Localized Correction towards Conditional Quantile}
\ziyang{Move to appendix}
As shown in Eq \eqref{eqn:localized_band}, the final upper and lower bounds can be viewed as a two-step correction: 1. correction with localized score in training set; 2. correction with empirical quantile of the decorrelated score.

We now focus on the details of the localized correction in the first step.
Suppose we get access to a fixed model of $\hat{q}$ (in our algorithm, $\hat{q} = \hat{\mu}$).
% \qq{do we need to introduce a new notation $\hat q$ here?}
Consider
\begin{equation}\label{eqn:localized_correction}
    \hat{q}_{\alpha,h}(x) = \hat{q}(x) + \Q(\alpha, \hat{F}_h(E|X=x)),
\end{equation}
where $E = Y - \hat{q}(X)$.
Then the function $\hat{q}_{\alpha,h}(x)$ is actually corrected towards the conditional quantile function of $q_{\alpha}(x) = \inf_{y\in \R}[\P(Y\leq y|X=x)\geq \alpha]$.
More formally we express it as the following theorem.
\begin{thm}\label{thm:doubly_robust}
    Define $F_h(E=e|X=x) = \E[w_h(X|x)\mathds{1}_{e\leq Y-\hat{q}(X)}]$ as the population distribution of $\hat{F}_h$ and its corresponding population version of $\hat{q}_{\alpha,h}$ is defined as
    \begin{equation}
        \hat{q}_{\alpha, h}(x) = \hat{q}(x) + \Q(\alpha, F_h(E|X=x)),~\forall h > 0,
    \end{equation}
    we have:
    \begin{enumerate}
        \item If $\hat{q} = {q}_{\alpha}$, then ${q}_{\alpha,h} = {q}_{\alpha},~\forall h>0$.
        \item The right limitation of $q_{\alpha,h}$ at point $0$ converge to $q_\alpha$:
        $$
            \lim_{h\to 0^+}{q}_{\alpha, h}(x) = {q}_{\alpha}(x),~\forall x.
        $$
    \end{enumerate}
\end{thm}
% \qq{need to analyze the variance as well in the end.}
% \qq{acknowledge that this is infintie data and finite data has variance.}

From Theorem~\ref{thm:doubly_robust} we can see that the corrected model achieves double robustness 
% \qq{tricky. it can be worse than both in practice due to the variance?} 
in the sense that if either the model is accurate or the kernel density estimation is accurate to represent the conditional distribution, then our estimator is consistent.
In practice, the correction term of empirical quantile is evaluated on finite training data, we cannot pick infinitesimal $h$ to achieve the best performance since it has large variance.
Similar to kernel density estimation, the tradeoff between bias and variance can guide us the selection of the bandwidth $h$; see \citet{yu1998local} for more discussions on bandwidth selection.

==> tex/theory.tex <==
% \section{Theory: Statistical Results}

% \subsection{Asymptotic Results}

% \subsection{Non-Asymptotic Results}
% Given an estimate quantile model $\hat{q}_{\alpha}$, 
% we can similarly correct the quantile model as:
% \begin{equation}\label{eqn:quantile_correction}
%     q_{\alpha,h}(x_0) = \hat{q}_{\alpha}(x_0) + {\rm Quantile}(\alpha, \E[w_h(X|x_0)\delta_{(Y-\hat{q}_{\alpha}(X))}]),
% \end{equation}


\section{Theoretical Analysis}
In this section, we assume the non-conformity score $V$ is given,
and the estimation of $\hat{F}_h(V|X=x)$ is under i.i.d. samples from $(V_i,X_i)\sim P_{V,X}$.
In real world scenario, the conformity score is actually dependent with the samples $V_i, X_i$ 
since $V$ is often computed by the estimation residual by the training data $\{Y_i, X_i\}$,
and we reuse the information of $X_i$ in the training data unless we choose $V = Y$.
But for the simplicity of analysis, we assume samples $X_i$ does not effect the choice of $V$.

Since $\hat{F}_h(V|X=x)$ is the famous NW estimator, 
we have the following result describing the plug-in quantile estimator of $\hat{F}_h(V|X=x)$
if we compare with the true conditional quantile function $q_\alpha(x) = \inf\{v: F(v|X=x)\geq \alpha\}$.
% \begin{lem}
% About $|\hat{F}_h - F|$
% \end{lem}

\begin{pro}
Suppose 
About the plug-in quantile estimator $|\Q(\alpha, \hat{F}_h) - q_\alpha(x)|$
\end{pro}

\begin{cor}
Lipschitz, $h\to 0$, $n\to \infty$, we have $\P(V\leq \Q(\alpha, \hat{F}_h)) \to \alpha$.
\end{cor}

\begin{thm}
When $V$ is already good:
\begin{enumerate}
    \item $V$ is independent to $X$, then XXX
    \item $V = Y - q_\alpha(X)$, then $\Q(\alpha, F_h) \to 0$.
\end{enumerate}
\end{thm} 
